Extensions and restrictions of holomorphic foliations

We prove an extension criterion for codimension one foliations on projective hypersurfaces based on the degree of the foliation and the degree of the hypersurface, and we ensure, in some instances, an isomorphism between the corresponding spaces of foliations. We also present some examples of foliations that do not satisfy the extension criterion and do not extend.

==> 4extensoessobrehipersuperficies.tex <==
\section{Proof of the Theorem B}

 Let $\omega\in H^0(\X, \Omega^1_X(k))$ be a Pfaff equation determining $\F$. Let $\alpha\in H^0(\Pj^n,\Omega^1_{\Pj^n}(k))$ be a extension of $\omega$. If $\alpha$ is non-integrable, that is, $\alpha\wedge d\alpha\in H^0(\Pj^n,\Omega^3_{\Pj^n}(2k))$ is not null, then $\X$ is invariant by this $3$-form and by \ref{Poincaré problem} we have $\deg(\X)\leq 2k-3$, which is absurd.
\begin{comment}
If $k\geq 3$, \cite[Theorem B]{MR1452431} guarantees $\deg(\X)\leq 2k-3$, which is a absurd. Now, if $k=2$, we have $\alpha\wedge d\alpha$ generating degree zero foliation by curves on $\Pj^4$, i.e., a pencil of lines and $\X$ must be a hyperplane or it has a singular point. 

For $n>4$, let $\alpha\in H^0(\Pj^n,\Omega_{\Pj^n}^1(k))$ be an extension of $\omega$. To verify that $\alpha$ is integrable, it is sufficient to show that its restriction to a generic 4-dimensional hyperplane in $\Pj^n$ is integrable. 

Since $\X$ is smooth, for $\Hp\simeq \Pj^4$ generic hyperplane contained in $\Pj^n$, the Bertini's Theorem guarantees that $\X'=\X\cap \Hp$ is smooth hypersurface in $\Hp$ invariant by the restriction of $\alpha\wedge d\alpha$ to $\Hp$ and $\deg(\X')=\deg(\X)$. It follows from the proof in the case $n=4$ that the restriction of $\alpha$ is integrable. As $\Hp\simeq \Pj^4$ is generic, we have that $\alpha$ is integrable and it defines foliation over $\Pj^n$. So $\F$ extends.
\end{comment}

